MVD-Fusion: Single-view 3D via Depth-consistent Multi-view Generation

We present MVD-Fusion: a method for single-view 3D inference via generative modeling of multi-view-consistent RGB-D images. While recent methods pursuing 3D inference advocate learning novel-view generative models, these generations are not 3D-consistent and require a distillation process to generate a 3D output. We instead cast the task of 3D inference as directly generating mutually-consistent multiple views and build on the insight that additionally inferring depth can provide a mechanism for enforcing this consistency. Specifically, we train a denoising diffusion model to generate multi-view RGB-D images given a single RGB input image and leverage the (intermediate noisy) depth estimates to obtain reprojection-based conditioning to maintain multi-view consistency. We train our model using large-scale synthetic dataset Obajverse as well as the real-world CO3D dataset comprising of generic camera viewpoints. We demonstrate that our approach can yield more accurate synthesis compared to recent state-of-the-art, including distillation-based 3D inference and prior multi-view generation methods. We also evaluate the geometry induced by our multi-view depth prediction and find that it yields a more accurate representation than other direct 3D inference approaches.

==> figures/diffusion-vis.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{example-image-duck}
    \caption{{Multi-view 2.5D Diffusion}. Figure showing colored point cloud diffusion.}
    \figlabel{nvs-gso-fig}
\end{figure*}

==> figures/nvs-gso.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{media/vis_gso.pdf}
    \caption{Qualitative results on novel view synthesis. We compare our method with Zero123 and SyncDreamer on the Google Scanned Objects dataset. \shubham{is there a bug here? Z123 and SyncD look the same!}} 
    \figlabel{nvs-gso-fig}
\end{figure*}

==> figures/nvs-obja.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{media/vis_obja.pdf}
    \caption{Qualitative results on novel view synthesis. We compare our method with Zero123 and SyncDreamer on the Objaverse dataset. \shubham{is there a bug here? Z123 and SyncD look the same!}}
    \figlabel{nvs-obja-fig}
\end{figure*}

==> tables/abla-obja.tex <==
\begin{table}[t]
\renewcommand\arraystretch{0.9}
\begin{center}
\caption{Ablation study on Objaverse furniture test set. We see that depth models}% \TODO{...} %\shubham{let's remove depth=1, and instead add Ours w/o CFG}}
\begin{tabularx}{8cm}{p{2.5cm}X<{\centering}X<{\centering}X<{\centering}}
\toprule[1.5pt]
Method  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS  $\downarrow$\\
\midrule[1pt]
%\midrule[1pt]
Voxel       & 20.76 & 0.852 & 0.135 \\
Depth-1     & 20.57 & 0.843 & 0.139 \\
Depth-3     & 20.29 & 0.843 & 0.146 \\
Depth-5     & 20.50 & 0.848 & 0.138 \\
\bottomrule[1.5pt]
\end{tabularx}
\end{center}
%\vspace{-2mm}

%\vspace{-5mm}
\tablelabel{abla-obja}
\end{table}

